Differentially Private Histograms in the Shuffle Model from Fake Users

There has been much recent work in the shuffle model of differential privacy, particularly for approximate $d$-bin histograms. While these protocols achieve low error, the number of messages sent by each user -- the message complexity -- has so far scaled with $d$ or the privacy parameters. The message complexity is an informative predictor of a shuffle protocol's resource consumption. We present a protocol whose message complexity is two when there are sufficiently many users. The protocol essentially pairs each row in the dataset with a fake row and performs a simple randomization on all rows. We show that the error introduced by the protocol is small, using rigorous analysis as well as experiments on real-world data. We also prove that corrupt users have a relatively low impact on our protocol's estimates.

==> old_step3.tex <==
The final algorithm in our sequence is $\cB_{m,q}$. When used as a post-processing of $\cR_{2,q}(x)$, it simulates the behavior of $\cC_{m,2,q}(x)$. This is because it samples the counts of messages produced by the $m$ executions of $\cR_{2,q}(00)$ and outputs a random set of messages obeying those counts (updated to include the input message).

As with the previous arguments, if $\cB_{m,q}$ were differentially private then $\cC_{m,2,q}$ would be differentially private. But it happens that we only need to prove privacy for one pair of inputs (instead of all pairs):

\begin{algorithm}
\caption{$\cB_{m,q}$}
\label{alg:binomial}

\KwIn{$y \in \zo^2$}
\KwOut{$\vec{y} \in (\zo^2)^*$}

$t \sim \Bin(m, 2q(1-q))$

$c_{01} \sim \Bin(t,1/2)$

$c_{10} \gets t-c_{01}$

$c_{11} \sim \Bin(m-t,q^2/(q^2 + (1-q)^2))$

$c_{00} \gets m-t-c_{11}$

$c_y \gets c_y + 1$

Sample $\vec{y}$, a uniformly random list of binary strings such that $c_y$ counts the frequency of $y$

\Return{$\vec{y}$}
\end{algorithm}

\begin{clm}
If $\cB_{m,q}$ is $(\eps,\delta)$-differentially private for inputs from $\cX_2 = \{01,10\}$, then $\cC_{m,2,q}$ is $(\eps,\delta)$-differentially private for inputs from $\cX_2$.
\end{clm}
\begin{proof}
Our goal is to use
\begin{align}
\pr{}{\cB_{m,q}(01) \in Y} &\leq e^\eps \cdot \pr{}{\cB_{m,q}(10) \in Y} + \delta \label{eq:bmq-1}\\
\pr{}{\cB_{m,q}(10) \in Y} &\leq e^\eps \cdot \pr{}{\cB_{m,q}(01) \in Y} + \delta \label{eq:bmq-2},
\end{align}
%\eqref{eq:bmq-1} and \eqref{eq:bmq-2}
to prove that
\begin{align}
\pr{}{\cC_{m,2,q}(01) \in Y} &\leq e^\eps \cdot \pr{}{\cC_{m,2,q}(10) \in Y} + \delta \label{eq:cm2q-1}\\
\pr{}{\cC_{m,2,q}(10) \in Y} &\leq e^\eps \cdot \pr{}{\cC_{m,2,q}(01) \in Y} + \delta \label{eq:cm2q-2},
\end{align}
Without loss of generality, we will focus on proving \eqref{eq:cm2q-1}.

We first compute the probability mass functions of $\cR_{2,q}(10), \cR_{2,q}(01), \cR_{2,q}(00)$:%the behavior of $\cC_{m,2,q}(01)$. By construction, the output is one sample from $\cR_{2,q}(01)$ shuffled with $m$ independent samples from $\cR_{2,q}(00)$. We plot 
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c||c|}
    \hline
         & $\cR_{2,q}(10)$ & $\cR_{2,q}(01)$ & $\cR_{2,q}(00)$ \\ \hline
         00 & $q(1-q)$ & $q(1-q)$ & $(1-q)^2$ \\ \hline
         01 & $q^2$ & $(1-q)^2$ & $q(1-q)$ \\ \hline
         10 & $(1-q)^2$ & $q^2$ & $q(1-q)$ \\ \hline
         11 & $q(1-q)$ & $q(1-q)$ & $q^2$ \\ \hline
    \end{tabular}
    \caption{Probability mass functions of three distributions $\cR_{2,q}(10), \cR_{2,q}(01), \cR_{2,q}(00)$}
    \label{tab:pmf}
\end{table}

Next, we argue that $\cC_{m,2,q}(01)$ has the same distribution over $(\zo^2)^*$ as $\cB_{m,q}(\cR_{2,q}(01))$. In both, one message is generated from $\cR_{2,q}(01)$ and shuffled with $m$ other messages, so we direct our attention to those other messages. In $\cC_{m,2,q}(01)$, they are sampled i.i.d. from $\cR_{2,q}(00)$. Referring to Table \ref{tab:pmf}, observe that number of messages of value $01$ or $10$ is distributed as $\Bin(m,2q(1-q))$. And, conditioned on a message being $01$ or $10$, either value is equally likely. This is captured by the distribution of $c_{01}$ and $c_{10}$ in $\cB_{m,q}(\cR_{2,q}(01))$. Meanwhile, the probability that a message has value $11$ conditioned on not being either $01$ or $10$ is $q^2 / (q^2 + (1-q)^2)$; this is captured by the distribution of $c_{11}$.

We finally prove \eqref{eq:cm2q-1} using the equivalence $\cC_{m,2,q}(01) = \cB_{m,q}(\cR_{2,q}(01))$ and Table \ref{tab:pmf}:
\begin{align*}
&\pr{}{\cC_{m,2,q}(01) \in Y} \\
={}& \pr{}{\cB_{m,q}(\cR_{2,q}(01)) \in Y} \\
={}& \pr{}{\cB_{m,q}(00) \in Y } \cdot \pr{}{\cR_{2,q}(01) = 00} + \pr{}{\cB_{m,q}(01) \in Y } \cdot \pr{}{\cR_{2,q}(01) = 01} \\
&+ \pr{}{\cB_{m,q}(10) \in Y } \cdot \pr{}{\cR_{2,q}(01) = 10} + \pr{}{\cB_{m,q}(11) \in Y } \cdot \pr{}{\cR_{2,q}(01) = 11} \\
={}& \pr{}{\cB_{m,q}(00) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 00} + \pr{}{\cB_{m,q}(01) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 10} \\
&+ \pr{}{\cB_{m,q}(10) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 01} + \pr{}{\cB_{m,q}(11) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 11} \\
\leq{}& \pr{}{\cB_{m,q}(00) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 00} + (e^\eps \cdot \pr{}{\cB_{m,q}(10) \in Y } + \delta) \cdot \pr{}{\cR_{2,q}(10) = 10} \\
&+ (e^\eps \cdot \pr{}{\cB_{m,q}(01) \in Y } + \delta) \cdot \pr{}{\cR_{2,q}(10) = 01} + \pr{}{\cB_{m,q}(11) \in Y } \cdot \pr{}{\cR_{2,q}(10) = 11} \\
\leq{}& e^\eps \cdot \pr{}{\cC_{m,2,q}(10) \in Y} + \delta
\end{align*}
The third equality comes from observing that the probability mass function for $\cR_{2,q}(10)$ is the same as that of $\cR_{2,q}(01)$ except for one swap. The first inequality comes from \eqref{eq:bmq-1} and \eqref{eq:bmq-2}.
\end{proof}

Finally, we argue that the algorithm is private when $m$ and $q$ obey a certain condition.
\begin{clm}
If $mq(1-q) \geq 20 \cdot \left( \tfrac{e^\eps+1}{e^\eps-1}\right)^2 \cdot  \ln\left(\tfrac{2}{\delta} \right)$, then $\cB_{m,q}$ is $(\eps,2\delta)$-differentially private for inputs from $\{01,10\}$.
\end{clm}
\begin{proof}
By a multiplicative Chernoff bound, we have that $t \geq \ex{}{t}/2 = mq(1-q)$ with probability $1-\delta$. The remainder of the proof conditions on this event.

If the input of $\cB_{m,q}$ has value either $01$ or $10$, observe that the joint distribution of $(c_{00},c_{11})$ is completely independent of the input. Also note that $c_{01} + c_{10} = t+1$ with probability 1 on either input (the plus one comes from the step $c_y \gets c_y +1$). This means \eqref{eq:bmq-1} and \eqref{eq:bmq-2} hold so long as the algorithm $\ind{y=01} + \Bin(t,1/2)$ is $(\eps,\delta)$-differentially private. By Lemma \ref{lem:b_noise} and our bound on $t$, it suffices for $mq(1-q) \geq 20 \cdot \left( \tfrac{e^\eps+1}{e^\eps-1}\right)^2 \cdot  \ln\left(\tfrac{2}{\delta} \right)$. 
\end{proof}
